Revisiting Physically Realizable Adversarial Object Attack against LiDAR-based Detection: Clarifying Problem Formulation and Experimental Protocols

Adversarial robustness in LiDAR-based 3D object detection is a critical research area due to its widespread application in real-world scenarios. While many digital attacks manipulate point clouds or meshes, they often lack physical realizability, limiting their practical impact. Physical adversarial object attacks remain underexplored and suffer from poor reproducibility due to inconsistent setups and hardware differences. To address this, we propose a device-agnostic, standardized framework that abstracts key elements of physical adversarial object attacks, supports diverse methods, and provides open-source code with benchmarking protocols in simulation and real-world settings. Our framework enables fair comparison, accelerates research, and is validated by successfully transferring simulated attacks to a physical LiDAR system. Beyond the framework, we offer insights into factors influencing attack success and advance understanding of adversarial robustness in real-world LiDAR perception.

==> fig/fig_asr_scatter.tex <==
\newcommand{\lossAblationScatterPlot}[5]{
\begin{tikzpicture}
\begin{axis}[height=.35\columnwidth,width=.45\columnwidth,
	xlabel=#1,ylabel=#2, 
        ymin=#3, ymax=#4,
        xmin=10,xmax=60,
        scatter/classes={
            pointpillar={color={rgb,255:red,31;green,119;blue,180}},  
            pointrcnn={color={rgb,255:red,255;green,127;blue,14}},      
            pointrcnn_s1={mark=square*, color={rgb,255:red,44;green,160;blue,44}}, 
            voxel_rcnn_car={color={rgb,255:red,214;green,39;blue,40}},
            voxel_rcnn_car_s1={mark=square*, color={rgb,255:red,148;green,103;blue,189}},
            pvrcnn={color={rgb,255:red,140;green,86;blue,75}},
            second={color={rgb,255:red,227;green,119;blue,194}}
        }]
]
    \addplot[
        scatter,only marks,
        scatter src=explicit symbolic
    ]
    table[meta=label] {#5};
    
    % \addlegendentry{PointPillar}
    % \addlegendentry{PointRCNN}
    % \addlegendentry{$\text{PointRCNN}_\text{Stage-1}$}
    % \addlegendentry{Voxel-RCNN}
    % \addlegendentry{$\text{Voxel-RCNN}_\text{Stage-1}$}
    % \addlegendentry{PV-RCNN}
    % \addlegendentry{SECOND}
\end{axis}
\end{tikzpicture}
}

\newcommand{\transferabilityScatterPlot}[4]{
\begin{tikzpicture}
\begin{axis}[height=.35\columnwidth,width=.45\columnwidth,
	xlabel=#1,  
        ymin=#2, ymax=#3,
        xmin=10,xmax=60,
        scatter/classes={
            pointpillar={color={rgb,255:red,31;green,119;blue,180}},  
            pointrcnn={color={rgb,255:red,255;green,127;blue,14}},      
            pointrcnn_s1={mark=square*, color={rgb,255:red,44;green,160;blue,44}}, 
            voxel_rcnn_car={color={rgb,255:red,214;green,39;blue,40}},
            voxel_rcnn_car_s1={mark=square*, color={rgb,255:red,148;green,103;blue,189}},
            pvrcnn={color={rgb,255:red,140;green,86;blue,75}},
            second={color={rgb,255:red,227;green,119;blue,194}}
        }]
]
    \addplot[
        scatter,only marks,
        scatter src=explicit symbolic
    ]
    table[meta=label] {#4};
    
    % \addlegendentry{PointPillar}
    % \addlegendentry{PointRCNN}
    % \addlegendentry{$\text{PointRCNN}_\text{Stage-1}$}
    % \addlegendentry{Voxel-RCNN}
    % \addlegendentry{$\text{Voxel-RCNN}_\text{Stage-1}$}
    % \addlegendentry{PV-RCNN}
    % \addlegendentry{SECOND}
\end{axis}
\end{tikzpicture}
}



\begin{figure}[htp]
\centering
\begin{tabular}{c c}
\lossAblationScatterPlot{}{V}{1.2}{2.0}{fig/loss_ablation_scatter/projected_volume_vs_bev_asr.csv}
& \transferabilityScatterPlot{}{1.2}{2.0}{fig/transferability_scatter/projected_volume_vs_bev_asr.csv}   \\ 
\lossAblationScatterPlot{}{$\text{V}_\text{Proj}$}{0}{1.5}{fig/loss_ablation_scatter/volume_vs_3d_asr.csv}
& \transferabilityScatterPlot{}{0}{1.5}{fig/transferability_scatter/volume_vs_3d_asr.csv}   \\ 
\lossAblationScatterPlot{}{$L_2$}{0}{6.5}{fig/loss_ablation_scatter/l2_norm_vs_3d_asr.csv}
& \transferabilityScatterPlot{}{0}{6.5}{fig/transferability_scatter/l2_norm_vs_3d_asr.csv}   \\ 
\lossAblationScatterPlot{Accuracy (BEV/3D)}{$\mathcal{L}$}{0}{0.2}{fig/loss_ablation_scatter/laplacian_vs_3d_asr.csv}
& \transferabilityScatterPlot{Accuracy (BEV/3D)}{0}{0.2}{fig/transferability_scatter/laplacian_vs_3d_asr.csv}   \\ 
\end{tabular}
\caption{The figure presents a 4x2 grid of plots illustrating the ASR across different metrics of the adversarial meshes: Volume ($V$), Projected volume ($\text{V}_\text{Proj}$), $L_2$ norm and Laplacian loss ($\mathcal{L}$). The first row shows the ASR for BEV mAP, while other rows show the ASR for 3D mAP. The first column represents white-box attacks, and the second column demonstrates transfer attacks across all metrics.}
\label{fig:sphere-level}
\end{figure}

==> tab/transferNetwork-black.tex <==
\begin{table*}[]
    \centering
\scriptsize
\setlength{\tabcolsep}{4pt}
    \begin{tabular}{ll ccccc}
    \toprule
       &  & 
PointPillar~\cite{lang2019pointpillars}&
PointRCNN~\cite{shi2019pointrcnn}&
PV-RCNN~\cite{shi2020pv}&
Voxel RCNN~\cite{deng2021voxel}&
SECOND~\cite{yan2018second}  \\\midrule
\mr{2}{Baseline}&Clean& 77.57&78.67&84.37&85.66&88.72\\
&Vanilla& 57.18&66.60&66.23&76.10&73.95\\\midrule
one-stage&PointPillar~\cite{lang2019pointpillars} & &&&&\\\midrule
\mr{3}{two-stage:first stage}&PointRCNN~\cite{shi2019pointrcnn}   & &&&&\\  
&PV-RCNN~\cite{shi2020pv} & &&&&\\
&Voxel RCNN~\cite{deng2021voxel} & &&&&\\\midrule
\mr{3}{two-stage: second stage}&PointRCNN~\cite{shi2019pointrcnn}   & &&&&\\  
&PV-RCNN~\cite{shi2020pv} & &&&&\\
&Voxel RCNN~\cite{deng2021voxel} & &&&&\\
\bottomrule
    \end{tabular}
    \caption{The transferability of the black-box adversarial mesh attack is evaluated by generating the adversarial mesh based on the surrogate model listed in the columns, targeting \textbf{PointPillar}, testing it on the models shown in the rows.}
    \label{tab:black-box-transferability-pp}
\end{table*}

% \begin{table*}[]
%     \centering
%     \scriptsize
% \setlength{\tabcolsep}{4pt}
%     \begin{tabular}{ll ccccc}
%     \toprule
%        &  & 
% PointPillar~\cite{lang2019pointpillars}&
% PointRCNN~\cite{shi2019pointrcnn}&
% PV-RCNN~\cite{shi2020pv}&
% Voxel RCNN~\cite{deng2021voxel}&
% SECOND~\cite{yan2018second}  \\\midrule
% \mr{2}{Baseline}&Clean& 77.57&78.67&84.37&85.66&88.72\\
% &Vanilla& 57.18&66.60&66.23&76.10&73.95\\\midrule
% one-stage&PointPillar~\cite{lang2019pointpillars} & &&&&\\\midrule
% \mr{3}{two-stage:first stage}&PointRCNN~\cite{shi2019pointrcnn}   & &&&&\\  
% &PV-RCNN~\cite{shi2020pv} & &&&&\\
% &Voxel RCNN~\cite{deng2021voxel} & &&&&\\\midrule
% \mr{3}{two-stage: second stage}&PointRCNN~\cite{shi2019pointrcnn}   & &&&&\\  
% &PV-RCNN~\cite{shi2020pv} & &&&&\\
% &Voxel RCNN~\cite{deng2021voxel} & &&&&\\
% \bottomrule
%     \end{tabular}
%     \caption{The transferability of the black-box adversarial mesh attack is evaluated by generating the adversarial mesh based on the surrogate model listed in the columns, targeting \textbf{PointRCNN}, testing it on the models shown in the rows.}
%     \label{tab:black-box-transferability-pr}
% \end{table*}

% \begin{table*}[]
%     \centering
%     \scriptsize
% \setlength{\tabcolsep}{4pt}
%     \begin{tabular}{ll ccccc}
%     \toprule
%        &  & 
% PointPillar~\cite{lang2019pointpillars}&
% PointRCNN~\cite{shi2019pointrcnn}&
% PV-RCNN~\cite{shi2020pv}&
% Voxel RCNN~\cite{deng2021voxel}&
% SECOND~\cite{yan2018second}  \\\midrule
% \mr{2}{Baseline}&Clean& 77.57&78.67&84.37&85.66&88.72\\
% &Vanilla& 57.18&66.60&66.23&76.10&73.95\\\midrule
% one-stage&PointPillar~\cite{lang2019pointpillars} & &&&&\\\midrule
% \mr{3}{two-stage:first stage}&PointRCNN~\cite{shi2019pointrcnn}   & &&&&\\  
% &PV-RCNN~\cite{shi2020pv} & &&&&\\
% &Voxel RCNN~\cite{deng2021voxel} & &&&&\\\midrule
% \mr{3}{two-stage: second stage}&PointRCNN~\cite{shi2019pointrcnn}   & &&&&\\  
% &PV-RCNN~\cite{shi2020pv} & &&&&\\
% &Voxel RCNN~\cite{deng2021voxel} & &&&&\\
% \bottomrule
%     \end{tabular}
%     \caption{The transferability of the black-box adversarial mesh attack is evaluated by generating the adversarial mesh based on the surrogate model listed in the columns, targeting \textbf{PV-RCNN}, testing it on the models shown in the rows.}
%     \label{tab:black-box-transferability-pv}
% \end{table*}

==> tab/white_box_compare.tex <==

\begin{table}[]
    \centering
    \scriptsize
\setlength{\tabcolsep}{1pt}
    \begin{tabular}{l |cc|cc|cc|cc|cc}
    \toprule
        \mr{2}{Method}& 
\multicolumn{2}{c|}{PP~\cite{lang2019pointpillars}}&
\multicolumn{2}{c|}{PR~\cite{shi2019pointrcnn}}&
\multicolumn{2}{c|}{PVR~\cite{shi2020pv}}&
\multicolumn{2}{c|}{VR~\cite{deng2021voxel}}&
\multicolumn{2}{c}{SC~\cite{yan2018second} } \\\cmidrule{2-11}
 &BEV &3D Box&BEV &3D Box&BEV &3D Box&BEV &3D Box&BEV &3D Box\\\midrule
% Clean& 86.76 &77.57& 85.67 &78.67& 88.92 &84.37& 89.15 &85.66& 88.72&81.82\\

Vanilla& 7.09 & 26.29 & 10.16 & 15.34 & 6.53 & 21.50 & 1.18 & 11.16 & 1.31 & 9.62 \\
% 80.61 & 57.18& 76.97&66.60& 83.11&66.23& 88.10 &76.10& 87.56&73.95\\
PhyAdv
% 77.65 &53.83& 72.35&60.64& 86.67&78.08& 77.25 &67.17& 85.82&71.46\\
% & 10.50 & 30.60 & 15.55 & 22.92 & 2.53 & 7.46 & 13.35 & 21.59 & 3.27 & 19.45 \\
&	12.20 &	36.25 &	15.50 &	22.35 &	2.34 &	6.99 &	13.11 &	21.47 &	3.34 &	12.66 \\
\rowcolor{yellow!10}
MR(\ref{eq:full-loss-logit})
% & 12.64 & 55.45 & 14.23 & 20.54 & 14.36 & 33.31 & 14.85 & 30.71 & 7.90 & 25.14 
&	\textbf{23.58} &	\textbf{44.26} &	\textbf{26.74} &	\textbf{37.30} &	8.60 &	30.69 &	\textbf{15.04} &	\textbf{29.83} &	\textbf{7.77} &	17.15 
 
\\
% 75.79 &34.56  & 73.48 & 62.51  & 76.15 & 56.27 & 75.91& 59.35& 81.71 &66.42  \\
\rowcolor{yellow!10}
MR(\ref{eq:full-loss1})
% & 14.03 & 45.89 & 14.95 & 22.61 & 6.34 & 17.89 & 14.48 & 25.37 & 7.99 & 24.83
&	23.25 &	43.95 &	23.89 &	35.22 &	\textbf{13.99} &	\textbf{31.98} &	15.03 &	29.79 &\textbf{	7.77} &	\textbf{17.45}  
\\
% 74.59 & 41.97 & 72.86 & 60.88 & 83.28 & 69.28 & 76.24 &  63.93 & 81.63 & 66.69\\ 
   \bottomrule

    \end{tabular}
    \caption{Attacks performance in white-box setting. }
    \label{tab:baseline}
\end{table}
